TSDM: A Scheduling Policy for Joint Throughput-AoI Optimization in Multichannel Wireless Networks

Optimizing for both low Age of Information (AoI) and high throughput is critical for remote sensing applications that rely on multichannel wireless networks. However, jointly optimizing these two metrics is an analytically challenging problem, particularly in systems with heterogeneous and unreliable channels. To address this challenge, we propose TSDM, a Two-Stage Deficit Matching scheduling framework. TSDM is based on a second-order approach that characterizes the performance of each data flow by its mean and temporal variance. In the first stage, TSDM translates the high-level utility maximization objective into a concrete set of target mean and temporal variance statistics for transmissions over each node-channel pair. In the second stage, a low-complexity Weighted Matching Deficit (WMD) rule performs real-time channel assignment. We theoretically prove that TSDM achieves the desired mean and temporal variance for each flow. Furthermore, we conduct extensive simulations on two open joint throughput-AoI optimization problems. In both cases, TSDM significantly outperforms existing scheduling policies.

==> specialcase.tex <==
\section{OPTIMALITY OF THE TSDM POLICY UNDER NODE-SYMMETRIC CHANNELS}

In this section, we study homogeneous node case where $p_{ij}=p_j$ for all $i\in\mathcal{I}$ and $j\in\mathcal{J}$. 
This corresponds to a node-symmetric setting in which all nodes experience the same channel reliability on a given channel, while the reliabilities may still vary across different channels. 

Under this assumption, we show that our proposed TSDM policy is optimal.
Let $\mu_i[\eta]$ and $\sigma_i^2[\eta]$ denote the throughput and 
temporal variance of node $i$ under an arbitrary scheduling policy $\eta$. 
We show that under TSDM, the achieved $\mu_i$ and $\sigma_i^2$ satisfy 
$\mu_i = \mu_i[\eta]$ and $\sigma_i^2 \leq \sigma_i^2[\eta]$ for all $i$.

Consider the following process as a random variable $S(t)$:
\[
S(t)
= \sum_{i=1}^{N} Z_i(t)
  - \mathbb{E}\!\Biggl[\sum_{i=1}^{N} Z_i(t)\Biggr]
= \sum_{i=1}^{N} \bigl(Z_i(t) - \mathbb{E}[Z_i(t)]\bigr),
\]
where the last equality follows from the linearity of expectation.

Since $\{S(t)\}$ are i.i.d. random variables, we have:
\begin{align*}
    \mathbb{E}[S(t)] &= 0,\\[2pt]
    \mathrm{Var}(S(t)) &= \sigma_{\text{tot}}^2
        = \sum_{j=1}^{M} \bigl(p_j - p_j^2\bigr),
\end{align*}
where the variance is identical for all nodes at each channel~$j$.

Furthermore, we can express the variance of $S$ as:
\begin{align}
\operatorname{Var}(S)
&= \operatorname{Var}\!\left(\sum_{i=1}^{N} (Z_i-\mathbb{E}[Z_i])\right) \nonumber\\
&= \operatorname{Var}\!\left(\sum_{i=1}^{N} Z_i\right) \nonumber\\
&= \sum_{i=1}^{N}\Var(Z_i)
   + 2\sum_{1\le i<k\le N}\Cov(Z_i,Z_k).
   \label{eq:var-sum-ik}
\end{align}

According to the Cauchy–Schwarz inequality, for any pair $(i,k)$: $\bigl|\operatorname{Cov}(Z_i,Z_k)\bigr|
  \le \sqrt{\operatorname{Var}(Z_i)\,\operatorname{Var}(Z_k)}
  = \sigma_i\sigma_k.$

Then, we get:
\[
\operatorname{Var}(S)=\sigma_{\text{tot}}^2
  \le \sum_{i=1}^{N}\sigma_i^{2}
    + 2\sum_{1\le i<k\le N}\sigma_i\sigma_k
  = \Bigl(\sigma_1+\sigma_2+\dots+\sigma_N\Bigr)^2.
\]

Taking the square root of both sides gives:$\sigma_{\text{tot}}
  \le
  \sum_{i=1}^{N}\sigma_i.$
Therefore,
\begin{align}
  \sum_{i=1}^{N}\sigma_i
  \;\ge\;
  \sigma_{\text{tot}}
  = \sqrt{\sum_{j=1}^{M}\bigl(p_j - p_j^2\bigr)}.
  \label{eq:outerbound}
\end{align}
This constraint must hold for all the scheduling policies under this setting. 

Then we analyze the performance of our scheduling policy. According to Eq.~\eqref{eq:somean2} and Eq.~\eqref{eq:sovariance2}, we have $ \sum_{i=1}^{N}\sigma_{ij}= \sqrt{p_j - p_j^2}.$
Let  $\sigma_{ij}=\lambda_i\sqrt{\,p_j - p_j^2\,}  ,\forall j$ and $\lambda_{i}\ge 0,\sum_{i=1}^N \lambda_{i}=1$.

Then according condition Eq.~\eqref{eq:sumofvariance} in first stage, we have: $\sigma_i=\lambda_i\sqrt{\sum_{j=1}^M (p_j-p_j^2)}.$ And using $\sum_{i=1}^N \lambda_i = 1$, we obtain:
\begin{align}\label{eq:innerbound}
    \sum_{i=1}^N \sigma_i
=\sqrt{\sum_{j=1}^M (p_j-p_j^2)}.
\end{align}
Under the proposed policy, the constraint bound in Eq.~\eqref{eq:outerbound} is achieved with equality, as shown in \eqref{eq:innerbound}, implying that the bound is tight. Moreover, TSDM satisfies all constraints specified in Section~\ref{section:policy}. Therefore, the proposed policy is optimal in this special case.




% \begin{remark}[Tightness of the Outer Bound]
% The inequality in~\eqref{eq:outerbound} provides a universal lower bound on 
% the aggregate standard deviation $\sum_i \sigma_i$. 
% In the homogeneous case where $p_{ij}=p_j$, 
% we can explicitly construct $\{\sigma_{ij}\}$ such that the equality holds, 
% and hence the outer bound is tight. 
% For general heterogeneous channels with $p_{ij}$ varying across nodes, 
% the equality condition of the Cauchy--Schwarz inequality cannot be satisfied in general. 
% Consequently, the bound in~\eqref{eq:outerbound} is typically not tight, 
% and the minimum achievable variance is strictly larger than $\sigma_{\text{tot}}$.
% \end{remark}



 



